Social Processes: Probabilistic Meta-learning for Adaptive Multiparty Interaction Forecasting

Adaptively forecasting human behavior in social settings is an important step toward achieving Artificial General Intelligence. Most existing research in social forecasting has focused either on unfocused interactions, such as pedestrian trajectory prediction, or on monadic and dyadic behavior forecasting. In contrast, social psychology emphasizes the importance of group interactions for understanding complex social dynamics. This creates a gap that we address in this paper: forecasting social interactions at the group (conversation) level. Additionally, it is important for a forecasting model to be able to adapt to groups unseen at train time, as even the same individual behaves differently across different groups. This highlights the need for a forecasting model to explicitly account for each group's unique dynamics. To achieve this, we adopt a meta-learning approach to human behavior forecasting, treating every group as a separate meta-learning task. As a result, our method conditions its predictions on the specific behaviors within the group, leading to generalization to unseen groups. Specifically, we introduce Social Process (SP) models, which predict a distribution over future multimodal cues jointly for all group members based on their preceding low-level multimodal cues, while incorporating other past sequences of the same group's interactions. In this work we also analyze the generalization capabilities of SP models in both their outputs and latent spaces through the use of realistic synthetic datasets.

==> ablations_means_table_haggling.tex <==
\begin{table*}[!htb]
% \vspace{-30pt}
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Mean (Std.) Errors in Predicted Means for the Ablation Experiments with the SP-uniform GRU Model.} The reported mean and std. are over sequences in the Haggling Test Sets. Lower is better for all except for speaking status accuracy.}
\label{tab:ablations-means-haggling}

\begin{subtable}[t]{\textwidth}
\caption{\textbf{Random Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lccccc@{}}
\toprule
  & & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} & \textbf{Speaking} \\
  & & MSE (cm) & MSE (cm) & MAE (\degree) & MAE (\degree) & Accuracy \\

\midrule
   \textbf{Full Model} & & 15.84~(5.5) & 17.76~(7.5) & 20.65~(19.9) & 21.73~(29.5) & 0.671~(0.22) \\
   
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{2}{*}{\textbf{Encoding Partner Behavior}}
  & no-pool & 18.20~(6.7) & 18.05~(7.7) & 16.76~(12.8) & 14.30~(20.9) & 0.690~(0.21) \\
  & pool-oT & 17.02~(6.1) & 19.18~(6.5) & 23.71~(25.1) & 17.80~(26.8) & 0.738~(0.21) \\ [1ex]

  \multirow{2}{*}{\textbf{No Deterministic Decoding}}
  & Shared Social Encoders   & 15.76~(7.2) & 16.34~(6.6) & 45.54~(44.6) & 21.87~(25.0) & 0.644~(0.22) \\
  & Unshared Social Encoders & 17.40~(6.9) & 18.33~(6.7) & 18.62~(14.7) & 14.54~(20.2) & 0.704~(0.23) \\
\bottomrule
\end{tabular*}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth}
\caption{\textbf{Fixed-Initial Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lccccc@{}}
\toprule
  & & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} & \textbf{Speaking} \\
  & & MSE (cm) & MSE (cm) & MAE (\degree) & MAE (\degree) & Accuracy \\

\midrule
   \textbf{Full Model} & & 16.53~(6.0) & 18.20~(8.0) & 20.74~(19.5) & 21.31~(28.9) & 0.674~(0.22) \\
   
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{2}{*}{\textbf{Encoding Partner Behavior}}
  & no-pool & 18.64~(6.7) & 18.45~(7.4) & 16.85~(12.9) & 14.29~(20.5) & 0.687~(0.21) \\
  & pool-oT & 17.39~(6.2) & 18.97~(6.4) & 23.90~(24.6) & 17.63~(25.6) & 0.730~(0.21) \\ [1ex]

  \multirow{2}{*}{\textbf{No Deterministic Decoding}}
  & Shared Social Encoders   & 16.93~(8.1) & 17.15~(7.0) & 45.49~(44.3) & 21.83~(24.7) & 0.637~(0.22) \\
  & Unshared Social Encoders & 18.54~(7.9) & 19.18~(7.1) & 18.68~(14.9) & 14.44~(20.0) & 0.700~(0.23) \\
\bottomrule
\end{tabular*}
\end{subtable}
\end{table*}


==> ablations_means_table_mnm.tex <==
\begin{table*}[!htb]
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Mean (Std.) Errors in Predicted Means for the Ablation Experiments with the SP-uniform GRU Model.} The reported mean and std. are over sequences in the MatchNMingle Test Sets. Lower is better.}
\label{tab:ablations-means-mnm}

\begin{subtable}[t]{\textwidth}
\caption{\textbf{Random Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lcccc@{}}
\toprule
  & & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} \\
  & & MSE (px) & MSE (px) & MAE (\degree) & MAE (\degree) \\

\midrule
  \textbf{Full Model} & & 41.48~(22.2) & 37.82~(18.9) & 56.39~(47.8) & 62.59~(54.3) \\
   
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{2}{*}{\textbf{Encoding Partner Behavior}}
  & no-pool & 36.25~(19.3) & 30.88~(18.1) & 47.28~(39.0) & 62.09~(54.5) \\
  & pool-oT & 41.81~(19.7) & 33.78~(17.9) & 54.01~(45.3) & 63.32~(54.8) \\ [1ex]

  \multirow{2}{*}{\textbf{No Deterministic Decoding}}
  & Shared Social Encoders   & 41.84~(19.9) & 30.99~(18.4) & 44.59~(37.2) & 72.02~(62.4) \\
  & Unshared Social Encoders & 37.25~(19.7) & 36.13~(18.0) & 62.81~(55.6) & 56.15~(52.6) \\
\bottomrule
\end{tabular*}
\end{subtable}
\vspace{0pt}

\begin{subtable}[t]{\textwidth}
\caption{\textbf{Fixed-Initial Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lcccc@{}}
\toprule
  & & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} \\
  & & MSE (px) & MSE (px) & MAE (\degree) & MAE (\degree) \\

\midrule
   \textbf{Full Model} & & 42.75~(21.7) & 42.18~(19.8) & 57.79~(48.6) & 64.44~(53.3) \\
   
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{2}{*}{\textbf{Encoding Partner Behavior}}
  & no-pool & 36.17~(17.4) & 31.77~(16.5) & 48.28~(39.6) & 64.19~(53.3) \\
  & pool-oT & 41.91~(18.6) & 34.17~(16.0) & 54.95~(45.7) & 65.20~(53.7) \\ [1ex]

  \multirow{2}{*}{\textbf{No Deterministic Decoding}}
  & Shared Social Encoders   & 41.29~(18.2) & 31.62~(16.9) & 45.54~(38.0) & 73.30~(60.9) \\
  & Unshared Social Encoders & 37.78~(18.5) & 35.28~(16.3) & 63.96~(56.1) & 58.23~(53.0) \\
\bottomrule
\end{tabular*}
\end{subtable}
\end{table*}


==> ablations_nll_table.tex <==
\begin{table*}[!t]
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Mean (Std.) LL for the Ablation Experiments with the SP-uniform GRU Model.} The reported mean and std. are over individual sequences in the test sets. Higher is better.}
\label{tab:ablations-nll}

\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lcccc@{}}
\toprule
  & & \multicolumn{2}{c}{\textbf{MatchNMingle}} & \multicolumn{2}{c}{\textbf{Haggling}} \\
  \cmidrule{3-6}
  & & \textbf{Random} & \textbf{Fixed-Initial} & \textbf{Random} & \textbf{Fixed-Initial} \\
  
\midrule
  \textbf{Full Model} & & 87.0~(38.4) & 85.5~(38.3) & 79.9~(50.5) & 78.6~(52.2) \\
  
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{2}{*}{\textbf{Encoding Partner Behavior}}
  & no-pool & 77.8~(31.2) & 76.9~(31.0) & 54.5~(75.5) & 50.1~(97.5) \\
  & pool-oT & 82.3~(33.3) & 81.0~(33.6) & 66.9~(26.0) & 66.8~(25.7) \\ [1ex]

  \multirow{2}{*}{\textbf{No Deterministic Decoding}} 
  & Shared Social Encoders   & 88.5~(40.7) & 87.6~(39.6) & 93.1~(39.3) & 91.9~(40.4) \\
  & Unshared Social Encoders & 81.4~(38.1) & 80.2~(37.8) & 66.6~(24.0) & 64.8~(23.4) \\
\bottomrule
\end{tabular*}
\end{table*}


==> hparams_table.tex <==
\begin{table}[!htb]
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Architecture Hyperparameters for real-world behavior dataset experiments (MnM / Haggling).} For the meta-learning models, the number of parameters are reported for the simplest \textit{-latent} variant.}
\label{tab:hparams}

\begin{tabular}[b]{@{}lccccc@{}}
\toprule
  \textbf{Hyperparameter} & \textbf{VED-MLP} & \textbf{VED-GRU} & \textbf{NP} & \textbf{SP-MLP} & \textbf{SP-GRU} \\

\midrule
  \textbf{Sequence Encoder/Decoder} \\
    \hspace{3mm}Number of layers        & $2$ & $1$ & $2$ & $2$ & $1$ \\
    \hspace{3mm}Hidden dim              & $180$ & $320$ & $180/460$ & $64$ & $320$ \\
  \textbf{Partner Pooler $\psi(\bm{x}_j)$} \\
    \hspace{3mm}Number of MLP layers    & \textemdash & \textemdash & \textemdash & $2$ & $2$ \\
    \hspace{3mm}MLP hidden dim          & \textemdash & \textemdash & \textemdash & $64$ & $64$ \\
    \hspace{3mm}Output dim              & \textemdash & \textemdash & \textemdash & $32$ & $32$ \\
  \textbf{$\bm{z}$ Encoder} \\
    \hspace{3mm}Number of layers        & $2$ & $2$ & $2$ & $2$ & $2$ \\
    \hspace{3mm}Hidden dim              & $64$ & $64$ & $64$ & $64$ & $64$ \\
  \textbf{Representations} \\
    \hspace{3mm}$\bm{e}$, $\bm{r}$, $\bm{s}$, $\bm{z}$ dim  & $64$ & $64$ & $64$ & $64$ & $64$ \\
  \textbf{Multi-Head Attention} \\
    \hspace{3mm}Query/Key dim           & \textemdash & \textemdash & $32$ & $32$ & $32$ \\
    \hspace{3mm}Number of heads         & \textemdash & \textemdash & $8$ & $8$ & $8$ \\

\midrule
  \textbf{Number of parameters} \\
  \hspace{3mm}MatchNMingle Dataset &  $254$K & $1.1$M & $274$K & $283$K & $3.0$M \\
  \hspace{3mm}Haggling Dataset &  $711$K & $1.1$M & $2.8$M & $2.2$M & $3.0$M \\
\bottomrule
\end{tabular}
\end{table}


==> means_table_haggling.tex <==
\begin{table*}[!htb]
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Mean (Std.) Errors in Predicted Means over Sequences in the Haggling Test Sets.} Lower is better for all metrics except for speaking status accuracy. Underline indicates best measure within family.}
\label{tab:mean-errors-haggling}

\begin{subtable}[h]{\textwidth}
\caption{\textbf{Random Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lccccc@{}}
\toprule
  \multirow{2}{*}{\textbf{Family}} & \multirow{2}{*}{\textbf{Model}} & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} & \textbf{Speaking} \\
  & & MSE (cm) & MSE (cm) & MAE (\degree) & MAE (\degree) & Accuracy \\

\midrule
  \multirow{2}{*}{\textbf{VED \cite{haNeuralRepresentationSketch2017, bowmanGeneratingSentencesContinuous2016}}}
  & VED-MLP & 42.04~(16.0) & 41.53~(15.6) & 24.70~(20.7) & 19.02~(13.3) & 0.636~(0.24) \\
  & VED-GRU & \underline{0.79}~(0.4) & \underline{0.75}~(0.4) & \underline{1.55}~(0.6) & \underline{1.06}~(0.4) & \underline{0.989}~(0.02) \\
  
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{NP \cite{garneloNeuralProcesses2018, kimAttentiveNeuralProcesses2019}}}
  & NP-latent & 14.21~(6.5) & 15.06~(6.1) & 16.29~(13.8) & 12.82~(13.7) & 0.787~(0.23) \\
  & NP-uniform & 15.01~(7.3) & 15.97~(7.2) & 17.45~(18.3) & 14.65~(20.0) & 0.715~(0.24) \\
  & ANP-dot & \underline{11.86}~(5.4) & \underline{12.22}~(5.5) & \underline{15.44}~(13.3) & \underline{12.56}~(18.0) & \underline{0.806}~(0.23) \\
  & ANP-mh & 16.36~(7.4) & 17.17~(7.2) & 19.41~(20.4) & 16.02~(22.1) & 0.692~(0.21) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{Ours (SP-MLP)}}
  & SP-latent & 25.58~(10.1) & \underline{26.57}~(9.0) & 91.07~(23.9) & 97.09~(22.5) & 0.638~(0.08) \\
  & SP-uniform & 31.99~(8.2) & 36.33~(7.3) & 91.08~(23.9) & 91.36~(23.9) & 0.629~(0.18) \\
  & ASP-dot & 27.16~(7.7) & 31.19~(7.1) & 90.88~(23.9) & 91.43~(23.8) & 0.704~(0.19) \\
  & ASP-mh & \underline{23.88}~(7.8) & 27.13~(7.7) & \underline{90.50}~(23.9) & \underline{91.04}~(24.1) & \underline{0.792}~(0.24) \\ [1ex]
  
  \multirow{4}{*}{\textbf{Ours (SP-GRU)}}
  & SP-latent & 17.18~(6.5) & 17.41~(6.2) & \underline{17.76}~(15.8) & \underline{14.78}~(20.7) & 0.713~(0.23) \\
  & SP-uniform & 15.84~(5.5) & 17.76~(7.5) & 20.65~(19.9) & 21.73~(29.5) & 0.671~(0.22) \\
  & ASP-dot & 22.59~(8.7) & 23.52~(10.2) & 17.90~(11.3) & 16.10~(19.3) & 0.722~(0.24) \\
  & ASP-mh & \underline{14.65}~(5.8) & \underline{15.38}~(6.1) & 28.06~(24.5) & 36.90~(37.9) & \underline{0.767}~(0.23) \\
\bottomrule
\end{tabular*}
\end{subtable}

\vfill
\vspace{7pt}

\begin{subtable}[h]{\textwidth}
\caption{\textbf{Fixed-Initial Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lccccc@{}}
\toprule
  \multirow{2}{*}{\textbf{Family}} & \multirow{2}{*}{\textbf{Model}} & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} & \textbf{Speaking} \\
  & & MSE (cm) & MSE (cm) & MAE (\degree) & MAE (\degree) & Accuracy \\

\midrule
  \multirow{2}{*}{\textbf{VED \cite{haNeuralRepresentationSketch2017, bowmanGeneratingSentencesContinuous2016}}}
  & VED-MLP & 41.71~(16.2) & 41.27~(15.8) & 24.36~(19.8) & 19.33~(13.4) & 0.640~(0.25) \\
  & VED-GRU & \underline{0.76}~(0.4) & \underline{0.72}~(0.3) & \underline{1.56}~(0.6) & \underline{1.04}~(0.3) & \underline{0.989}~(0.02) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{NP \cite{garneloNeuralProcesses2018, kimAttentiveNeuralProcesses2019}}}
  & NP-latent & 13.85~(6.1) & 14.71~(5.7) & 16.22~(14.1) & \underline{12.69}~(13.9) & \underline{0.774}~(0.24) \\
  & NP-uniform & 15.01~(7.5) & 15.95~(7.5) & 17.26~(15.9) & 14.68~(18.7) & 0.701~(0.24) \\
  & ANP-dot & \underline{12.83}~(5.9) & \underline{13.26}~(6.0) & \underline{16.19}~(13.7) & 13.56~(17.8) & 0.717~(0.23) \\
  & ANP-mh & 16.68~(7.9) & 17.43~(7.7) & 19.78~(21.2) & 15.57~(20.3) & 0.682~(0.21) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{Ours (SP-MLP)}}
  & SP-latent & 25.27~(10.0) & \underline{26.33}~(8.9) & 91.14~(23.8) & 97.09~(22.5) & 0.640~(0.09) \\
  & SP-uniform & 32.93~(9.4) & 37.16~(8.5) & 91.15~(23.9) & 91.36~(23.9) & 0.633~(0.18) \\
  & ASP-dot & 27.94~(7.8) & 31.83~(7.1) & 90.93~(23.9) & 91.43~(23.8) & 0.628~(0.20) \\
  & ASP-mh & \underline{24.07}~(8.1) & 27.35~(8.3) & \underline{90.53}~(23.9) & \underline{91.07}~(24.1) & \underline{0.770}~(0.25) \\ [1ex]
  
  \multirow{4}{*}{\textbf{Ours (SP-GRU)}}
  & SP-latent & 16.66~(6.2) & 17.17~(6.0) & \underline{17.67}~(16.0) & \underline{14.64}~(20.3) & \underline{0.705}~(0.23)   \\
  & SP-uniform & \underline{16.53}~(6.0) & 18.20~(8.0) & 20.74~(19.5) & 21.31~(28.9) & 0.674~(0.22)   \\
  & ASP-dot & 23.91~(8.8) & 25.34~(10.6) & 19.11~(12.8) & 17.36~(19.0) & 0.635~(0.26)  \\
  & ASP-mh & 16.87~(6.0) & \underline{16.96}~(6.1) & 28.90~(24.3) & 37.23~(37.6) & \underline{0.705}~(0.24) \\
\bottomrule
\end{tabular*}
\end{subtable}
\end{table*}


==> means_table_mnm.tex <==
\begin{table*}[!htb]
\ra{1.1}
\centering
\scriptsize
\caption{\textbf{Mean (Std.) Errors in Predicted Means over Sequences in the MatchNMingle Test Sets.} Lower is better. Underline indicates best measure within family.}
\label{tab:mean-errors-mnm}

\begin{subtable}[h]{\textwidth}
\caption{\textbf{Random Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lcccc@{}}
\toprule
  \multirow{2}{*}{\textbf{Family}} & \multirow{2}{*}{\textbf{Model}} & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} \\
  & & MSE (px) & MSE (px) & MAE (\degree) & MAE (\degree) \\

\midrule
  \multirow{2}{*}{\textbf{VED \cite{haNeuralRepresentationSketch2017, bowmanGeneratingSentencesContinuous2016}}}
  & VED-MLP & 131.12~(52.0) & 110.58~(45.3) & 74.84~(39.6) & 97.55~(56.8) \\
  & VED-GRU & \underline{30.00}~(18.0) & \underline{24.80}~(17.2) & \underline{22.62}~(15.7) & \underline{24.72}~(29.1) \\
  
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{NP \cite{garneloNeuralProcesses2018, kimAttentiveNeuralProcesses2019}}}
  & NP-latent & \underline{41.16}~(21.4) & \underline{33.41}~(21.1) & 25.58~(21.1) & 35.88~(47.7) \\
  & NP-uniform & 42.93~(20.9) & 39.76~(21.0) & 27.14~(21.4) & 38.22~(48.0) \\
  & ANP-dot & 41.59~(20.4) & 37.57~(19.5) & 26.42~(20.6) & 37.19~(47.6) \\
  & ANP-mh & 41.49~(20.7) & 36.77~(19.5) & \underline{25.39}~(20.7) & \underline{35.82}~(48.0) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{Ours (SP-MLP)}}
  & SP-latent & 297.24~(92.3) & 258.71~(87.8) & 95.11~(41.3) & 110.74~(51.6) \\
  & SP-uniform & 73.53~(34.2) & 61.95~(36.2) & \underline{95.00}~(41.3) & 110.06~(50.8) \\
  & ASP-dot & 78.86~(24.8) & 67.77~(21.7) & 95.02~(41.3) & 110.27~(51.1) \\
  & ASP-mh & \underline{63.99}~(22.4) & \underline{53.59}~(22.2) & \underline{95.00}~(41.3) & \underline{109.81}~(50.6) \\ [1ex]
  
  \multirow{4}{*}{\textbf{Ours (SP-GRU)}}
  & SP-latent & \underline{38.58}~(20.9) & \underline{27.45}~(19.9) & \underline{49.50}~(44.1) & 63.06~(57.4) \\
  & SP-uniform & 41.48~(22.2) & 37.82~(18.9) & 56.39~(47.8) & 62.59~(54.3) \\
  & ASP-dot & 44.17~(21.4) & 37.13~(19.7) & 55.41~(47.1) & 62.14~(54.5) \\
  & ASP-mh & 43.49~(21.3) & 38.29~(19.8) & 57.68~(47.3) & \underline{61.94}~(53.7) \\
\bottomrule
\end{tabular*}
\end{subtable}

\vfill

\vspace{6pt}

\begin{subtable}[h]{\textwidth}
\caption{\textbf{Fixed-Initial Context}}
\begin{tabular*}{\textwidth}{@{}l @{\extracolsep{\fill}} lcccc@{}}
\toprule
  \multirow{2}{*}{\textbf{Family}} & \multirow{2}{*}{\textbf{Model}} & \textbf{Head Loc.} & \textbf{Body Loc.} & \textbf{Head Ori.} & \textbf{Body Ori.} \\
  & & MSE (px) & MSE (px) & MAE (\degree) & MAE (\degree) \\
  
\midrule
  \multirow{2}{*}{\textbf{VED \cite{haNeuralRepresentationSketch2017, bowmanGeneratingSentencesContinuous2016}}}
  & VED-MLP & 131.67~(52.6) & 111.50~(46.0) & 75.97~(38.7) & 98.26~(55.6) \\
  & VED-GRU & \underline{29.51}~(16.5) & \underline{24.33}~(16.1) & \underline{22.75}~(15.9) & \underline{26.60}~(32.0) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{NP \cite{garneloNeuralProcesses2018, kimAttentiveNeuralProcesses2019}}}
  & NP-latent &  \underline{40.82}~(19.1) & \underline{32.81}~(19.5) & \underline{25.58}~(21.6) & \underline{38.97}~(51.0) \\
  & NP-uniform & 45.22~(19.1) & 40.60~(19.0) & 28.34~(22.4) & 42.65~(51.8) \\
  & ANP-dot & 44.67~(18.6) & 40.03~(18.2) & 29.08~(21.9) & 44.44~(54.4) \\
  & ANP-mh & 42.75~(18.7) & 37.56~(18.4) & 26.95~(22.3) & 42.20~(51.9) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multirow{4}{*}{\textbf{Ours (SP-MLP)}}
  & SP-latent & 296.36~(92.8) & 259.46~(87.5) & 94.75~(39.0) & 108.62~(47.3) \\
  & SP-uniform & 81.61~(40.7) & 64.44~(42.6) & 94.68~(39.0) & 108.26~(46.7) \\
  & ASP-dot & 92.03~(38.2) & 78.97~(33.1) & 94.69~(39.0) & 108.36~(46.9) \\
  & ASP-mh & \underline{66.22}~(25.5) & \underline{53.04}~(24.0) & \underline{94.67}~(39.0) & \underline{108.14}~(46.5) \\ [1ex]
  
  \multirow{4}{*}{\textbf{Ours (SP-GRU)}}
  & SP-latent & \underline{38.31}~(18.2) & \underline{26.79}~(17.7) & \underline{51.78}~(45.1) & 65.38~(55.9) \\
  & SP-uniform & 42.75~(21.7) & 42.18~(19.8) & 57.79~(48.6) & \underline{64.44}~(53.3) \\
  & ASP-dot & 54.42~(25.9) & 44.88~(22.6) & 56.12~(46.9) & 65.28~(54.5) \\
  & ASP-mh & 56.62~(26.3) & 47.78~(22.9) & 58.90~(47.9) & 64.46~(54.1) \\
\bottomrule
\end{tabular*}
\end{subtable}
\end{table*}


==> nll_table.tex <==
\centering
\scriptsize
\ra{1.14}
\setlength{\tabcolsep}{0.5pt}
\captionof{table}{\textbf{Mean (Std.) Log-Likelihood (LL) on the MatchNMingle and Haggling Test Sets.} For a single sequence, we sum over the feature and participant dimensions, and average over timesteps. The reported mean and std. are over individual sequences in the test sets. Higher is better. Underline indicates best LL within family.}
\label{tab:nll}

\begin{tabular}[b]{@{}lcccc@{}}
\toprule
  & \multicolumn{2}{c}{\textbf{MatchNMingle}} & \multicolumn{2}{c}{\textbf{Haggling}} \\
  \cmidrule{2-5}
  & \textbf{Random} & \textbf{Fixed-Initial} & \textbf{Random} & \textbf{Fixed-Initial} \\

\midrule
  \multicolumn{2}{@{}l}{\textbf{VED Family \cite{haNeuralRepresentationSketch2017, bowmanGeneratingSentencesContinuous2016}}} \\
  VED-MLP   & 8.1~(7.2) & 7.9~(7.0) & 4.0~(8.3) & 4.1~(8.2) \\
  VED-GRU   & 25.4~(18.0) & 25.1~(19.1) & 60.3~(2.2) & 60.3~(2.1) \\
  
\specialrule{\lightrulewidth}{1ex}{1ex}
  \multicolumn{2}{@{}l}{\textbf{NP Family \cite{garneloNeuralProcesses2018, kimAttentiveNeuralProcesses2019}}} \\
  NP-latent     & 22.1~(17.8) & \underline{21.6}~(18.5) & \underline{27.2}~(17.3) & \underline{27.9}~(16.3) \\
  NP-uniform    & 21.4~(18.8) & 20.5~(17.8) & 24.8~(22.9) & 25.0~(22.2) \\
  ANP-dot       & 22.8~(18.6) & 21.0~(18.3) & 26.7~(21.4) & 24.7~(20.8) \\
  ANP-mh        & \underline{23.6}~(15.6) & 20.0~(23.9) & 25.1~(23.1) & 24.8~(22.4) \\

\specialrule{\lightrulewidth}{1ex}{1ex}
  \multicolumn{2}{@{}l}{\textbf{Ours (SP-MLP)}} \\
  SP-latent     & 102.1~(29.9) & 101.5~(29.2) & 136.6~(7.0) & 136.7~(7.0) \\
  SP-uniform    & 112.8~(34.1) & \underline{111.4}~(33.8) & 138.3~(8.0) & 137.6~(8.4) \\
  ASP-dot       & 109.9~(32.9) & 107.6~(32.1) & 137.8~(7.5) & 136.4~(7.6) \\
  ASP-mh        & \underline{112.9}~(34.7) & 111.3~(33.6) & \underline{146.0}~(10.9) & \underline{145.7}~(10.2) \\ [1ex]

  \multicolumn{2}{@{}l}{\textbf{Ours (SP-GRU)}} \\
  SP-latent     & 86.4~(37.2) & 85.4~(37.2) & 66.7~(27.4) & 66.2~(30.7) \\
  SP-uniform    & 87.0~(38.4) & \underline{85.5}~(38.3) & \underline{79.9}~(50.5) & \underline{78.6}~(52.2) \\
  ASP-dot       & \underline{87.6}~(39.1) & 83.9~(38.1) & 38.4~(60.4) & 27.2~(93.4) \\
  ASP-mh        & 85.8~(37.1) & 82.3~(36.0) & 66.3~(30.3) & 59.3~(32.4) \\
\bottomrule
\end{tabular}

